FinePseudo: Improving Pseudo-Labelling through Temporal-Alignablity for Semi-Supervised Fine-Grained Action Recognition

Real-life applications of action recognition often require a fine-grained understanding of subtle movements, e.g., in sports analytics, user interactions in AR/VR, and surgical videos. Although fine-grained actions are more costly to annotate, existing semi-supervised action recognition has mainly focused on coarse-grained action recognition. Since fine-grained actions are more challenging due to the absence of scene bias, classifying these actions requires an understanding of action-phases. Hence, existing coarse-grained semi-supervised methods do not work effectively. In this work, we for the first time thoroughly investigate semi-supervised fine-grained action recognition (FGAR). We observe that alignment distances like dynamic time warping (DTW) provide a suitable action-phase-aware measure for comparing fine-grained actions, a concept previously unexploited in FGAR. However, since regular DTW distance is pairwise and assumes strict alignment between pairs, it is not directly suitable for classifying fine-grained actions. To utilize such alignment distances in a limited-label setting, we propose an Alignability-Verification-based Metric learning technique to effectively discriminate between fine-grained action pairs. Our learnable alignability score provides a better phase-aware measure, which we use to refine the pseudo-labels of the primary video encoder. Our collaborative pseudo-labeling-based framework `\textit{FinePseudo}' significantly outperforms prior methods on four fine-grained action recognition datasets: Diving48, FineGym99, FineGym288, and FineDiving, and shows improvement on existing coarse-grained datasets: Kinetics400 and Something-SomethingV2. We also demonstrate the robustness of our collaborative pseudo-labeling in handling novel unlabeled classes in open-world semi-supervised setups. Project Page: https://daveishan.github.io/finepsuedo-webpage/.

==> eccv_tables/abl_gauss_warp.tex <==
\setlength{\intextsep}{2pt} %
\begin{wraptable}{r}{0.5\textwidth} %
\arrayrulecolor{black}
\centering
\arrayrulecolor[rgb]{0.753,0.753,0.753}
\begingroup
\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{1.2pt}
\begin{tabular}{c!{\color{black}\vrule}c|c!{\color{black}\vrule}cc} 
\arrayrulecolor{black}\hline

\hline

\hline\\[-3mm]
\multirow{2}{*}{\textbf{SSL}} & \multicolumn{2}{c|}{\textbf{PennAction}} & \multicolumn{2}{c}{\textbf{Diving48}} \\
\arrayrulecolor[rgb]{0.753,0.753,0.753}\cline{2-3}
\multirow{2}{*}{\textbf{Objective}} & \textbf{Phase} & \textbf{Event} & \multirow{2}{*}{\textbf{10\%}} & \multirow{2}{*}{\textbf{20\%}} \\
& \textbf{Classi.} & \textbf{Progress} & & \\
\arrayrulecolor{black}\hline
w/o gaussian & 0.88 & 0.87 & 35.42 & 58.81 \\
with gaussian & \textbf{0.93} & \textbf{0.91} & \textbf{37.64} & \textbf{60.40} \\
\arrayrulecolor{black}\bottomrule
\end{tabular}
}
\endgroup
\vspace{-2mm}
\caption{Ablation: SSL pretraining of \( f_A \)}
\vspace{1mm}
\label{table:alignssl}
\end{wraptable}

